Factorized Fourier Neural Operators

We propose the Factorized Fourier Neural Operator (F-FNO), a learning-based approach for simulating partial differential equations (PDEs). Starting from a recently proposed Fourier representation of flow fields, the F-FNO bridges the performance gap between pure machine learning approaches to that of the best numerical or hybrid solvers. This is achieved with new representations - separable spectral layers and improved residual connections - and a combination of training strategies such as the Markov assumption, Gaussian noise, and cosine learning rate decay. On several challenging benchmark PDEs on regular grids, structured meshes, and point clouds, the F-FNO can scale to deeper networks and outperform both the FNO and the geo-FNO, reducing the error by 83% on the Navier-Stokes problem, 31% on the elasticity problem, 57% on the airfoil flow problem, and 60% on the plastic forging problem. Compared to the state-of-the-art pseudo-spectral method, the F-FNO can take a step size that is an order of magnitude larger in time and achieve an order of magnitude speedup to produce the same solution quality.

==> tables/context.tex <==
\begin{table}[t]
  \caption{Performance of \ac{F-FNO} on \TorusV and
  \TorusVF, with ablation studies to test the contribution of each context.
  Each result is accompanied by the
  standard deviation from three trials.}
  \begin{tabularx}{\linewidth}{Xr}
  \toprule
    & \multicolumn{1}{c}{N-MSE (\%)}   \\
  \midrule
  \TorusV \\
  \quad Without context & $43.8 \pm 0.9$\,\,\,  \\
  \quad With force  & $4.48 \pm 0.09 $ \\
  \quad With force and viscosity  & $2.06 \pm 0.02$ \\
  \midrule
  \TorusVF \\
  \quad Without context & $33.0 \pm 0.4 $\,\,\, \\
  \quad With force  & $ 4.2 \pm 0.1 $\,\,\, \\
  \quad With force and viscosity & $2.01 \pm 0.05$  \\
  \bottomrule
\end{tabularx}
\label{tab:mse_with_context}
\end{table}

